OfficeMate: Pilot Evaluation of an Office Assistant Robot

Office Assistant Robots (OARs) offer a promising solution to proactively provide in-situ support to enhance employee well-being and productivity in office spaces. We introduce OfficeMate, a social OAR designed to assist with practical tasks, foster social interaction, and promote health and well-being. Through a pilot evaluation with seven participants in an office environment, we found that users see potential in OARs for reducing stress and promoting healthy habits and value the robot's ability to provide companionship and physical activity reminders in the office space. However, concerns regarding privacy, communication, and the robot's interaction timing were also raised. The feedback highlights the need to carefully consider the robot's appearance and behaviour to ensure it enhances user experience and aligns with office social norms. We believe these insights will better inform the development of adaptive, intelligent OAR systems for future office space integration.

==> sections/5-conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
Our primary objectives were to develop and derive design insights from the functional prototype of an OAR system, OfficeMate, focusing on practical assistance, social interaction, navigation, and promoting health and well-being within a workplace environment. In our pilot study with seven participants, we explored the integration of OfficeMate in a real office setting, gathering insights on user experiences and perceptions. Participants appreciated the robot’s potential to encourage physical activities, provide mindfulness exercises, and alleviate stress, recognizing its role as a well-being reminder. The robot’s ability to engage in natural conversations and act as a companion was seen positively, enhancing motivation for well-being activities. However, participants highlighted concerns regarding privacy and monitoring, wary of potential misuse of personal data. They also noted the need for improvements in the robot’s movements, speed, conversational latency, and voice modulation to enhance safety and interaction flow. Future iterations of the OAR should focus on personalizing interactions, optimizing the timing of interventions to avoid disruptions, and balancing proactive engagement in well-being practices with users’ workflows. Addressing these considerations is essential for developing an effective and socially acceptable office assistant robot that supports employee well-being and productivity.
